Redundancy of information: lowering dimension

Let At denote the set of infinite sequences of effective dimension t. We determine both how close and how far an infinite sequence of dimension s can be from one of dimension t, measured using the Besicovitch pseudometric. We also identify classes of sequences for which these infima and suprema are realized as minima and maxima. When t < s, we find d(X,At) is minimized when X is a Bernoulli p-random, where H(p)=s, and maximized when X belongs to a class of infinite sequences that we call s-codewords. When s < t, the situation is reversed.

==> pgflibrarypatterns.meta.code.tex <==
% Copyright 2015 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\def\pgf@pat@type@uncolored{0}%
\def\pgf@pat@type@colored{1}%
\newif\ifpgf@pat@makepatternimmutable

\pgfkeys{/pgf/patterns/.cd,
  name/.store in=\pgf@pat@name,
  number ../.store in=\pgf@pat@number,
  type/.is choice,
    type/uncolored/.code={\let\pgf@pat@type=\pgf@pat@type@uncolored},
    type/colored/.code={\let\pgf@pat@type=\pgf@pat@type@colored},
    type/form only/.style={/pgf/patterns/type=uncolored},
    type/inherently colored/.style={/pgf/patterns/type=colored},
  x/.store in=\pgf@pat@xvec,
  y/.store in=\pgf@pat@yvec,
  parameters/.store in=\pgf@pat@parameters,
  defaults/.store in=\pgf@pat@defaults,
  append to defaults/.code={%
    \pgf@pat@addto@macro\pgf@pat@defaults{,#1}%
  },
  bottom left/.store in=\pgf@pat@bottomleft,
  top right/.store in=\pgf@pat@topright,
  tile size/.store in=\pgf@pat@tilesize,
  tile transformation/.store in=\pgf@pat@transformation,
  code/.store in=\pgf@pat@code,
  set up code/.store in=\pgf@pat@declarebefore,
  %
  name=,
  number ..=,
  type=uncolored,
  x=1cm, y=1cm,
  parameters=,
  defaults=,
  bottom left=,
  top right=,
  tile size=,
  tile transformation=,
  code=,
  set up code=,
}%

\def\pgf@pat@name@prefix{pgf@pattern@name@meta@}%

\def\pgfifpatternundefined#1{%
  \pgfutil@ifundefined{\pgf@pat@name@prefix#1}%
}%

\def\pgf@pat@adddef@to@macro#1#2{%
  \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter#1%
      \expandafter\expandafter\expandafter{\expandafter#1\expandafter%
        \def\expandafter#2\expandafter{#2}}%
}%

\def\pgf@pat@addto@macro#1#2{%
  \expandafter\def\expandafter#1\expandafter{#1#2}}%

\def\pgf@pat@process#1{%
  \pgf@process{#1}%
}%

\def\pgf@pat@doifnotempty#1{%
  \ifx#1\pgfutil@empty%
    \let\pgf@pat@next=\relax%
  \else%
    \let\pgf@pat@next=#1%
  \fi%
  \pgf@pat@next%
}%

\def\pgf@pat@processtransformations#1{#1}%
\def\pgf@pat@processpoint#1{%
  \pgf@process{#1}%
}%


\def\pgfdeclarepattern#1{%
  \begingroup%
    \nullfont%
    \def\pgf@pat@options{,#1}%
    \pgfkeys{/pgf/patterns/.cd,#1}%
    \ifx\pgf@pat@name\pgfutil@empty
        \pgferror{Declaring unnamed pattern}%
    \fi
    \ifx\pgf@pat@bottomleft\pgfutil@empty
        \pgferror{Bottom left corner of the bounding box unset}%
    \fi
    \ifx\pgf@pat@topright\pgfutil@empty
        \pgferror{Top right corner of the bounding box unset}%
    \fi
    \ifx\pgf@pat@tilesize\pgfutil@empty
        \pgferror{Tile size unset}%
    \fi
    \ifx\pgf@pat@code\pgfutil@empty
        \pgferror{Pattern code is empty}%
    \fi
    \pgf@declarepattern@meta%
  \endgroup%
}%
\def\pgf@declarepattern@meta{%
    \pgfifpatternundefined{\pgf@pat@name}{%
      \ifx\pgf@pat@parameters\pgfutil@empty%
        % No parameters, so pattern is declared now.
        \pgf@pat@declare%
        \edef\pgf@marshal{%
          \noexpand\pgf@pat@addto@macro\noexpand\pgf@pat@options{,number ..=\pgf@pattern@number}}%
        \pgf@marshal%
      \fi%
      % It is a bit inefficient that all the options for
      % immutable patterns are saved when only the type
      % and number are needed.
      \expandafter\global\expandafter\let\csname\pgf@pat@name@prefix\pgf@pat@name\endcsname=\pgf@pat@options%
    }{%
      \pgferror{Pattern `\pgf@pat@name' already defined}%
    }%
}%
\let\pgf@pat@declarebefore=\pgfutil@empty
\let\pgf@pat@declareafter=\pgfutil@empty
\let\pgf@pat@codebefore=\pgfutil@empty
\let\pgf@pat@codeafter=\pgfutil@empty

\def\pgf@pat@declare{%
   \pgfsysprotocol@getcurrentprotocol\pgf@pattern@temp%
   {%
     % Set up x and y vectors. Should use a scope rather than TeX group?
     % Vectors may be needed when the tile bounding box is
     % calculated.
     \pgfsetxvec{\pgfpoint{\pgf@pat@xvec}{+0pt}}%
     \pgfsetyvec{\pgfpoint{+0pt}{\pgf@pat@yvec}}%
     \pgf@pat@doifnotempty\pgf@pat@declarebefore%
     \pgfinterruptpath%
       \pgfpicturetrue%
       \pgf@relevantforpicturesizetrue%
       \pgftransformreset%
       \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
       \pgfsysprotocol@bufferedtrue%
       \pgfsys@beginscope%
         \pgfinterruptboundingbox%
           \pgfsetarrows{-}%
           \pgf@pat@doifnotempty\pgf@pat@codebefore
           \pgf@pat@code%
           \pgf@pat@doifnotempty\pgf@pat@codeafter%
         \endpgfinterruptboundingbox%
       \pgfsys@endscope%
       \pgfsysprotocol@getcurrentprotocol\pgf@pattern@code%
       \global\let\pgf@pattern@code=\pgf@pattern@code%
     \endpgfinterruptpath%
     \pgf@pat@doifnotempty\pgf@pat@declareafter%
     \pgf@pat@processpoint{\pgf@pat@bottomleft}%
     \pgf@xa=\pgf@x%
     \pgf@ya=\pgf@y%
     \pgf@pat@processpoint{\pgf@pat@topright}%
     \pgf@xb=\pgf@x%
     \pgf@yb=\pgf@y%
     \pgf@pat@processpoint{\pgf@pat@tilesize}%
     \pgf@xc=\pgf@x%
     \pgf@yc=\pgf@y%
     \begingroup%
       \pgftransformreset%
       \pgf@pat@processtransformations\pgf@pat@transformation%
       \pgfgettransformentries\aa\ab\ba\bb\shiftx\shifty%
       \global\edef\pgf@pattern@matrix{{\aa}{\ab}{\ba}{\bb}{\shiftx}{\shifty}}%
     \endgroup%
     % Now, build a name for the pattern
     \pgfutil@tempcnta=\pgf@pattern@number\relax%
     \advance\pgfutil@tempcnta by1\relax%
     \xdef\pgf@pattern@number{\the\pgfutil@tempcnta}%
     \xdef\pgf@marshal{\noexpand\pgfsys@declarepattern%
       {\pgf@pattern@number}%
       {\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}{\the\pgf@xc}{\the\pgf@yc}\pgf@pattern@matrix{\pgf@pattern@code}{\pgf@pat@type}}%
   }%
   \pgf@marshal%
   \pgfsysprotocol@setcurrentprotocol\pgf@pattern@temp%
}%

\def\pgf@pat@checkname#1{%
  \pgf@pat@@checkname#1[]\pgf@patstop}%

\def\pgf@pat@@checkname#1[#2]#3\pgf@patstop{%
  \def\pgf@pat@onlinename{#1}%
  \def\pgf@pat@onlineoptions{#2}%
}%


\def\pgf@pat@unravel#1/{%
  \pgfutil@ifnextchar\pgf@stop{\def\pgf@pat@unravelled{#1}}{\pgf@pat@unravel}}%

\pgfkeys{/handlers/.pattern/.code={%
    \expandafter\expandafter\expandafter\pgf@pat@unravel\pgfkeyscurrentpath/\pgf@stop%
    \pgfpatternalias{#1}{\pgf@pat@unravelled}%
}}%

\def\pgfpatternalias#1#2{%
  \begingroup%
    \pgf@pat@checkname{#1}%
    \expandafter\let\expandafter\pgf@pat@options\expandafter=%
      \csname\pgf@pat@name@prefix\pgf@pat@onlinename\endcsname%
    \pgf@pat@macroaskeys{/pgf/patterns/.cd}{\pgf@pat@options}%
    \pgfutil@toks@\expandafter{\pgf@pat@onlineoptions}%
    \edef\pgf@pat@tmp{append to defaults={\the\pgfutil@toks@}}%
    \expandafter\pgf@pat@addto@macro\expandafter\pgf@pat@options\expandafter{\expandafter,\pgf@pat@tmp}%
    \pgf@pat@addto@macro\pgf@pat@options{,name=#2}%
    \expandafter\global\expandafter\let\csname\pgf@pat@name@prefix#2\endcsname=\pgf@pat@options%
  \endgroup%
}%


\let\pgfsetfillpattern@old=\pgfsetfillpattern

\def\pgf@pat@macroaskeys#1#2{%
  \pgfutil@toks@\expandafter{#2}%
  \edef\pgf@marshal{\noexpand\pgfkeys{#1, \the\pgfutil@toks@}}%
  \pgf@marshal%
}%
\def\pgfsetfillpattern#1#2{%
  \pgf@pat@checkname{#1}%
  \pgfutil@ifundefined{\pgf@pat@name@prefix\pgf@pat@onlinename}{%
    \pgfsetfillpattern@old{\pgf@pat@onlinename}{#2}%
  }{%
    \let\pgf@pat@parameters=\pgfutil@empty%
    % Get pattern parameters, type, and number
    \expandafter\let\expandafter\pgf@pat@options\expandafter=%
      \csname\pgf@pat@name@prefix\pgf@pat@onlinename\endcsname%
    \pgf@pat@macroaskeys{/pgf/patterns/.cd}{\pgf@pat@options}%
    \ifx\pgf@pat@parameters\pgfutil@empty%
      % Immutable pattern. Do nothing.
    \else%
      % Mutable. Do a *lot*.
      \begingroup%
          \pgf@pat@macroaskeys{/pgf/pattern keys/.cd}{\pgf@pat@defaults}%
          \pgf@pat@macroaskeys{/pgf/pattern keys/.cd}{\pgf@pat@onlineoptions}%
          % ...to get the values of the current parameters...
          \edef\pgf@pat@current@parameters{\pgf@pat@parameters}%
          % ...and the internal pattern name.
          \edef\pgf@pat@onlinename{\pgf@pat@onlinename\pgf@pat@current@parameters}%
          \let\pgf@pat@name=\pgf@pat@onlinename%
          \pgfutil@ifundefined{\pgf@pat@name@prefix\pgf@pat@onlinename}{%
            %\ifpgf@pat@makepatternimmutable%
              \let\pgf@pat@parameters=\pgfutil@empty%
            %\fi%
            \pgf@declarepattern@meta%
          }{}%
          \expandafter%
        \endgroup%
        \expandafter\def\expandafter\pgf@pat@onlinename\expandafter{\pgf@pat@onlinename}%
        \expandafter\let\expandafter\pgf@pat@options\expandafter=%
      \csname\pgf@pat@name@prefix\pgf@pat@onlinename\endcsname%
      \pgf@pat@macroaskeys{/pgf/patterns/.cd}{\pgf@pat@options}%
    \fi%
    \ifx\pgf@pat@type\pgf@pat@type@uncolored%
      \pgf@pat@setpatternuncolored{\pgf@pat@number}{#2}%
    \else%
      \pgfsys@setpatterncolored{\pgf@pat@number}%
    \fi%
  }%
}%

\def\pgf@pat@setpatternuncolored#1#2{%
  \pgfutil@colorlet{pgf@tempcolor}{#2}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \pgfutil@extractcolorspec{pgf@tempcolor}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@pat@set@fill@patternuncolored\pgf@rgbcolor\relax{#1}%
}%
\def\pgf@pat@set@fill@patternuncolored#1,#2,#3\relax#4{%
  \pgfsys@setpatternuncolored{#4}{#1}{#2}{#3}%
}%

% Predefined patterns

\pgfdeclarepattern{
  name=Lines,
  parameters={
      \pgfkeysvalueof{/pgf/pattern keys/distance},
      \pgfkeysvalueof{/pgf/pattern keys/angle},
      \pgfkeysvalueof{/pgf/pattern keys/xshift},
      \pgfkeysvalueof{/pgf/pattern keys/yshift},
      \pgfkeysvalueof{/pgf/pattern keys/line width},
  },
  bottom left={%
    \pgfpoint
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  top right={%
    \pgfpoint
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  tile size={%
    \pgfpoint
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}%
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}},
  tile transformation={%
    \pgftransformrotate{\pgfkeysvalueof{/pgf/pattern keys/angle}}%
    \pgftransformshift{%
      \pgfpoint
        {\pgfkeysvalueof{/pgf/pattern keys/xshift}}%
        {\pgfkeysvalueof{/pgf/pattern keys/yshift}}}},
  defaults={
    distance/.initial=3pt,
    angle/.initial=0,
    xshift/.initial=0pt,
    yshift/.initial=0pt,
    line width/.initial=\the\pgflinewidth,
  },
  code={%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/pattern keys/line width}}%
    \pgfpathmoveto{\pgfpoint{-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}{0pt}}%
    \pgfpathlineto{\pgfpoint{.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}{0pt}}%
    \pgfusepath{stroke}%
  },
}

\pgfdeclarepattern{
  name=Hatch,
  parameters={
      \pgfkeysvalueof{/pgf/pattern keys/distance},
      \pgfkeysvalueof{/pgf/pattern keys/angle},
      \pgfkeysvalueof{/pgf/pattern keys/xshift},
      \pgfkeysvalueof{/pgf/pattern keys/yshift},
      \pgfkeysvalueof{/pgf/pattern keys/line width},
  },
  bottom left={%
    \pgfpoint
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  top right={%
    \pgfpoint
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  tile size={%
    \pgfpoint
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}%
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}},
  tile transformation={%
    \pgftransformrotate{\pgfkeysvalueof{/pgf/pattern keys/angle}}%
    \pgftransformshift{%
      \pgfpoint
        {\pgfkeysvalueof{/pgf/pattern keys/xshift}}%
        {\pgfkeysvalueof{/pgf/pattern keys/yshift}}}},
  defaults={
    distance/.initial=3pt,
    angle/.initial=0,
    xshift/.initial=0pt,
    yshift/.initial=0pt,
    line width/.initial=\the\pgflinewidth,
  },
  code={%
    \pgfsetlinewidth{\pgfkeysvalueof{/pgf/pattern keys/line width}}%
    \pgfpathmoveto{\pgfpoint{-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}{0pt}}%
    \pgfpathlineto{\pgfpoint{.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}{0pt}}%
    \pgfpathmoveto{\pgfpoint{0pt}{-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}}%
    \pgfpathlineto{\pgfpoint{0pt}{.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}}%
    \pgfusepath{stroke}%
  },
}

\pgfdeclarepattern{
  name=Dots,
  parameters={
      \pgfkeysvalueof{/pgf/pattern keys/distance},
      \pgfkeysvalueof{/pgf/pattern keys/angle},
      \pgfkeysvalueof{/pgf/pattern keys/xshift},
      \pgfkeysvalueof{/pgf/pattern keys/yshift},
      \pgfkeysvalueof{/pgf/pattern keys/radius},
  },
  bottom left={%
    \pgfpoint
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  top right={%
    \pgfpoint
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  tile size={%
    \pgfpoint
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}%
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}},
  tile transformation={%
    \pgftransformrotate{\pgfkeysvalueof{/pgf/pattern keys/angle}}%
    \pgftransformshift{%
      \pgfpoint
        {\pgfkeysvalueof{/pgf/pattern keys/xshift}}%
        {\pgfkeysvalueof{/pgf/pattern keys/yshift}}}},
  defaults={
    distance/.initial=3pt,
    angle/.initial=0,
    xshift/.initial=0pt,
    yshift/.initial=0pt,
    radius/.initial=.5pt,
  },
  code={%
    \pgfpathcircle%
      {\pgfpointorigin}%
      {\pgfkeysvalueof{/pgf/pattern keys/radius}}
    \pgfusepath{fill}%
  },
}

\pgfdeclarepattern{
  name=Stars,
  parameters={
      \pgfkeysvalueof{/pgf/pattern keys/distance},
      \pgfkeysvalueof{/pgf/pattern keys/angle},
      \pgfkeysvalueof{/pgf/pattern keys/xshift},
      \pgfkeysvalueof{/pgf/pattern keys/yshift},
      \pgfkeysvalueof{/pgf/pattern keys/radius},
      \pgfkeysvalueof{/pgf/pattern keys/points},
  },
  bottom left={%
    \pgfpoint
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {-.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  top right={%
    \pgfpoint
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}%
      {.5*(\pgfkeysvalueof{/pgf/pattern keys/distance})}},
  tile size={%
    \pgfpoint
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}%
      {\pgfkeysvalueof{/pgf/pattern keys/distance}}},
  tile transformation={%
    \pgftransformrotate{\pgfkeysvalueof{/pgf/pattern keys/angle}}%
    \pgftransformshift{%
      \pgfpoint
        {\pgfkeysvalueof{/pgf/pattern keys/xshift}}%
        {\pgfkeysvalueof{/pgf/pattern keys/yshift}}}},
  defaults={
    distance/.initial=3mm,
    angle/.initial=0,
    xshift/.initial=0pt,
    yshift/.initial=0pt,
    radius/.initial=1mm,
    points/.initial=5,
  },
  code={%
    \pgfmathsetmacro\a{180/(\pgfkeysvalueof{/pgf/pattern keys/points})}%
    \pgfpathmoveto{\pgfpointpolar{90}{\pgfkeysvalueof{/pgf/pattern keys/radius}}}%
    \foreach \i in {1,...,\pgfkeysvalueof{/pgf/pattern keys/points}}{%
        \pgfpathlineto{\pgfpointpolar{90+2*\i*\a-\a}{.5*(\pgfkeysvalueof{/pgf/pattern keys/radius})}}%
        \pgfpathlineto{\pgfpointpolar{90+2*\i*\a}{\pgfkeysvalueof{/pgf/pattern keys/radius}}}%
    }%
    \pgfpathclose%
    \pgfusepath{fill}%
  },
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> tikzlibrarypatterns.meta.code.tex <==
% Copyright 2015 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{patterns.meta}%

\tikzset{%
  pattern color/.code=\edef\tikz@pattern@color{#1},
  pattern/.code={%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillpattern{#1}{\tikz@pattern@color}}%
      \def\tikz@pattern{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
  }
}%

\def\tikz@pattern@color{black}%
\def\tikz@pattern{}%

\tikzset{patterns/.cd,
  .unknown/.code={%
    \let\tikz@pat@key=\pgfkeyscurrentname%
    \pgfkeys{/pgf/patterns/\tikz@pat@key/.try={#1}}%
  },
  bottom left/.style={/pgf/patterns/bottom left={\tikz@scan@one@point\pgf@pat@process#1}},
  top right/.style={/pgf/patterns/top right={\tikz@scan@one@point\pgf@pat@process#1}},
  bounding box/.style args={#1(#2)#3and#4(#5)#6}{%
    /tikz/patterns/bottom left={(#2)},
    /tikz/patterns/top right={#4(#5)},
  },
  tile size/.style={/pgf/patterns/tile size={\tikz@scan@one@point\pgf@pat@process#1}},
  tile transformation/.style={/pgf/patterns/tile transformation={%
      \let\tikz@transform=\relax\pgfkeys{/tikz/.cd,#1}}%
  },
  infer tile bounding box/.code={
    \def\pgf@pat@codeafter{%
      \xdef\tikz@pat@installbb{%
        \noexpand\pgfkeys{/tikz/patterns/bounding box={%
        (\the\pgf@picminx-#1,\the\pgf@picminy-#1) and
        (\the\pgf@picmaxx+#1,\the\pgf@picmaxy+#1)
      },
      /tikz/patterns/tile size={%
        (\the\pgf@picmaxx-\the\pgf@picminx,
          \the\pgf@picmaxy-\the\pgf@picminy)}}}%
    }%
    \let\pgf@pat@declarepost=\tikz@pat@installbb%
  },
  infer tile bounding box/.default=0pt,
}%

\def\tikzdeclarepattern#1{%
   \begingroup%
     \def\pgf@pat@codebefore{%
        \let\tikz@transform=\relax%
        \pgftransformreset% <- Hmm?
        \tikz@declarepattern@install%
        \ifnum\pgf@pat@type=0\relax%
          \let\pgfsetstrokecolor=\pgfutil@gobble%
          \let\pgfsetfillcolor=\pgfutil@gobble%
        \fi%
        \def\tikz@fig{%
          \tikzerror{You cannot use nodes inside a pattern}%
        }%
        \tikzset{pattern/.code={\tikzerror{You cannot nest patterns}},
          pattern color/.style={pattern}}%
     }%
     \pgfdeclarepattern{/tikz/patterns/.cd,#1}%
   \endgroup%
 }%

\def\tikz@declarepattern@install{%
  \let\tikz@compat@color@set=\tikz@compat@color@set@insidepatttern%
  \tikz@installcommands%
}%

\let\tikz@compat@color@set@orig=\tikz@compat@color@set
\def\tikz@compat@color@set@insidepatttern#1{%
  \tikz@compat@color@set@orig{#1}%
  \pgfsetfillcolor{#1}\pgfsetstrokecolor{#1}%
}%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

